Multi-agent LLM consultation increases agreement but weakens it as a deferral signal in medical question answering

In medical question answering, agreement among independently sampled answers can help determine when to defer to a clinician. Multi-agent consultation lets agents revise their answers after reading a report synthesised from their initial analyses, so the same report can influence multiple votes. We tested how consultation changes the ability of vote agreement to identify incorrect answers. For each of three open-weight models, we ran a nine-call consultation protocol on MedQA-USMLE and a 2,000-question subset of VM14K, a Vietnamese medical question-answering benchmark. We recorded every vote before and after consultation. Consultation increased unanimity in every model-benchmark setting and reduced the AUROC of vote agreement for detecting incorrect answers from 62-69 to 54-57, near the chance level of 50. Dissenting agents tended to adopt the initial majority answer even when it was incorrect, and a simulation showed that this alone is enough to explain the loss. On MedQA-USMLE, among answers that were unanimous after consultation, accuracy was 81-94% when the initial votes were unanimous and 58-63% when the initial votes were split 2-1. In additional experiments on the VM14K subset, the decline in AUROC persisted in a council of three different models and in a variant in which agents read one another's full analyses. These results support using agreement among pre-consultation votes to guide deferral.

==> tables/C_votes_medqa.tex <==
Qwen3-32B & 1.3--1.6 & 0.1--0.2 & 0.1--0.5 & 0.1 & -- & -- \\
Llama-3.3-70B & 1.6--1.8 & 0.1--0.2 & 0.4--0.6 & 0.1 & -- & -- \\
Llama-3.1-8B & 10.5--11.7 & 0.0--0.2 & 3.0--3.7 & 1.5--1.9 & -- & -- \\


==> tables/C_votes_sub.tex <==
Standard protocol, Qwen3-32B & 7.0--7.2 & 0.0--0.1 & 0.3--0.4 & 0.1 & -- & -- \\
Standard protocol, Llama-3.3-70B & 3.3--4.0 & 0.2--0.3 & 1.3 & 0.2--0.3 & -- & -- \\
Standard protocol, Llama-3.1-8B & 6.5--6.7 & 0.3--0.4 & 8.4--8.7 & 1.7--1.8 & -- & -- \\
Heterogeneous council & 1.8 & 0.1 & 16.8--17.9 & 0.5--0.6 & -- & -- \\
Consultation without report & 7.1--7.4 & 0.0--0.1 & 0.7--0.9 & 0.1 & -- & -- \\


==> tables/S_mad.tex <==
Qwen3-32B, VM14K & 9.6 & 26.0 & 66.0 & 66.4 & 86.3 & 17.6 & 24.0 & 58.9 & 57.9 \\
Llama-3.3-70B, VM14K & 19.9 & 20.2 & 65.0 & 57.2 & 79.9 & 15.3 & 22.8 & 60.9 & 59.4 \\
Qwen3-32B, MedQA-USMLE & 0.2 & 0.2 & 75.7 & 92.5 & 97.1 & 19.7 & 21.3 & 54.4 & 53.1 \\
Llama-3.1-8B, MedQA-USMLE & 6.3 & 1.8 & 60.1 & 47.9 & 55.2 & 10.8 & 14.3 & 64.2 & 63.2 \\

